Measurement of the charm mixing parameter $y_{CP} - y_{CP}^{K\pi}$ using two-body $D^0$ meson decays

A measurement of the ratios of the effective decay widths of $D^0 \to \pi^-\pi^+$ and $D^0 \to K^-K^+$ decays over that of $D^0 \to K^-\pi^+$ decays is performed with the LHCb experiment using proton-proton collisions at a centre-of-mass energy of $13 \, \mathrm{TeV}$, corresponding to an integrated luminosity of $6 \, \mathrm{fb^{-1}}$. These observables give access to the charm mixing parameters $y_{CP}^{\pi\pi} - y_{CP}^{K\pi}$ and $y_{CP}^{KK} - y_{CP}^{K\pi}$, and are measured as $y_{CP}^{\pi\pi} - y_{CP}^{K\pi} = (6.57 \pm 0.53 \pm 0.16) \times 10^{-3}$, $y_{CP}^{KK} - y_{CP}^{K\pi} = (7.08 \pm 0.30 \pm 0.14) \times 10^{-3}$, where the first uncertainties are statistical and the second systematic. The combination of the two measurements is $y_{CP} - y_{CP}^{K\pi} = (6.96 \pm 0.26 \pm 0.13) \times 10^{-3}$, which is four times more precise than the previous world average.

==> Authorship_LHCb-PAPER-2021-041-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abell{\'a}n Beteta,
F. Abudin{\'e}n,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C. Agapopoulou,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
G. Alkhazov,
P. Alvarez Cartelle,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
M. Andreotti,
D. Ao,
F. Archilli,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista de Souza Leite,
M. Barbetti,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
A. Bertolin,
C. Betancourt,
F. Betti,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
N.V. Biesuz,
S. Bifani,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
P. Campana,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
L. Carus,
K. Carvalho Akiba,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
S. Celani,
J. Cerasoli,
D. Cervenkov,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
L. Congedo,
A. Contu,
N. Cooke,
G. Coombs,
I. Corredoira ,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Dashkina,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
F. De Vellis,
J.A. de Vries,
C.T. Dean,
F. Debernardis,
D. Decamp,
V. Dedu,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Cicco,
P. Di Nezza,
S. Didenko,
L. Dieste Maronas,
S. Ding,
V. Dobishuk,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
L. Douglas,
A. Dovbnya,
A.G. Downes,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
J.M. Durham,
D. Dutta,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
L.N. Falcao,
Y. Fan,
B. Fang,
S. Farry,
D. Fazzini,
M. F{\'e}o,
A. Fernandez Prieto,
A.D. Fernez,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
A. Fkiaras,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
E. Gabriel,
G. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
L. Giambastiani,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
C. Giugliano,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
P. Gorbounov,
I.V. Gorelov,
C. Gotti,
J.P. Grabowski,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
B.R. Gruberg Cazon,
C. Gu,
M. Guarise,
M. Guittiere,
P. A. G{\"u}nther,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
J. Haimberger,
S.C. Haines,
T. Halewood-leagas,
P.M. Hamilton,
J.P. Hammerich,
Q. Han,
X. Han,
E.B. Hansen,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
K. Heijhoff,
K. Heinicke,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
R. Hou,
Y. Hou,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Iniukhin,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
X. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
Y. Kang,
M. Karacson,
D. Karpenkov,
M. Karpov,
J.W. Kautz,
F. Keizer,
D.M. Keller,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
J. Kubat,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
P. Li,
S. Li,
Y. Li,
Z. Li,
X. Liang,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
Q. Liu,
S. Liu,
A. Lobo Salvia,
A. Loi,
R. Lollini,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
S. L{\'o}pez Soli{\~n}o,
G.H. Lovell,
Y. Lu,
C. Lucarelli,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
L. Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
D. Maisuzenko,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
D. Manuzzi,
C.A. Manzari,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
J. Marks,
A.M. Marshall,
P.J. Marshall,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. Mcgrath,
N.T. Mchugh,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
G. Meier,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M. Milovanovic,
M.-N. Minard,
A. Minotti,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
R. Murta,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Normand,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
D.P. O'Hanlon,
S. Okamura,
R. Oldeman,
F. Oliva,
M.E. Olivares,
C.J.G. Onderwater,
R.H. O'Neil,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
O. Ozcelik,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
A. Pereiro Castro,
P. Perret,
M. Petric,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
T.T.H. Pham,
A. Philippov,
R. Piandani,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
F. Pisani,
M. Pizzichemi,
Resmi  P.K,
V. Placinta,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
V. Puill,
G. Punzi,
H. Qi,
W. Qian,
N. Qin,
R. Quagliani,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
R. Rajagopalan,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
R. Ribatti,
A.M. Ricci,
S. Ricciardi,
K. Rinnert,
P. Robbe,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
E.R.R. Rodriguez Rodriguez,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
M. Salomoni,
C. Sanchez Gras,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
O. Schneider,
A. Schopper,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
E.B. Shields,
Y. Shimizu,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
G. Simi,
S. Simone,
M. Singla,
N. Skidmore,
R. Skuza,
T. Skwarnicki,
M.W. Slater,
I. Slazyk,
J.C. Smallwood,
J.G. Smeaton,
E. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
S. Stone,
D. Strekalina,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
A.R. Tanner,
M.D. Tat,
A. Terentev,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
K.A. Thomson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
X. Tong,
D. Torres Machado,
D.Y. Tou,
E. Trifonova,
S.M. Trilov,
C. Trippl,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. van Beuzekom,
M. Van Dijk,
H. Van Hecke,
E. van Herwijnen,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Veronesi,
M. Vesterinen,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. Vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
K. Vos,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
N.K. Watson,
D. Websdale,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M. K. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
D. Yang,
S. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
A. Zharkova,
A. Zhelezov,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
X. Zhu,
X. Zhu,
Z. Zhu,
V. Zhukov,
Q. Zou,
S. Zucchelli,
D. Zuliani,
G. Zunica

==> my-symbols-def.tex <==
% sections numbered but not in TOC
% usage \toclesslab\section{title}{sect:a}
\newcommand{\nocontentsline}[3]{}
\newcommand{\tocless}[2]{\bgroup\let\addcontentsline=\nocontentsline#1{#2}\egroup}
\newcommand{\toclesslab}[3]{\bgroup\let\addcontentsline=\nocontentsline#1{#2\label{#3}}\egroup}

\usepackage{authblk}
\usepackage{enumitem}
\usepackage{placeins}

\usepackage{multirow}
\usepackage{booktabs}
\usepackage{dcolumn}
\usepackage{array}
\usepackage{rotating}

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF


\usepackage[separate-uncertainty]{siunitx}
\usepackage{physics}
\usepackage{bm}

%%% Parameters
%%%%%%%%%%%%%%%%%%%%%%% 

% analysis parameters
\def\mintime     {\ensuremath{0.45}}
\def\maxtime     {\ensuremath{8}}
\def\ipcut       {\ensuremath{\text{IP}(\Dz) < 60\mum}\xspace}
\def\notipcut    {\ensuremath{\text{IP}(\Dz) > 60\mum}\xspace}
\def\nbins       {\ensuremath{21}}

% numerical results (in 1e-4)
\def\agammaRSval  {\ensuremath{0.4}}
\def\agammaRSstat {\ensuremath{0.5}}
\def\agammaRSvalNoSecSubtr  {\ensuremath{0.1}}
\def\agammaRSstatNoSecSubtr {\ensuremath{0.5}}
\def\agammaRSsys  {\ensuremath{0.2}}
\def\agammaKKval  {\ensuremath{2.3}}
\def\agammaKKstat {\ensuremath{1.5}}
\def\agammaKKsys  {\ensuremath{0.3}}
\def\agammaPPval  {\ensuremath{4.0}}
\def\agammaPPstat {\ensuremath{2.8}}
\def\agammaPPsys  {\ensuremath{0.4}}
\def\agammaVal    {\ensuremath{2.7}}
\def\agammaStat   {\ensuremath{1.3}}
\def\agammaSys    {\ensuremath{0.3}}
\def\dAGammaVal   {\ensuremath{-1.7}}
\def\dAGammaStat  {\ensuremath{3.2}}
\def\dAGammaSys   {\ensuremath{0.2}}
\def\agammaCombVal    {\ensuremath{1.0}}
\def\agammaCombStat   {\ensuremath{1.1}}
\def\agammaCombSys    {\ensuremath{0.3}}
\def\PPagreementWithKKstatOnly {{\ensuremath{0.5\,\sigma}}\xspace}
\def\charmfitter    {\mbox{\textsc{CharmFitter}}\xspace}
\def\probmethod    {\mbox{\textsc{Prob}}\xspace}

\def\pvalueAGammaRSfitsRaw {{\ensuremath{7 \times 10^{-23}}}\xspace}
\def\pvalueAGammaRSfitsWeightedOne {{\ensuremath{45\%}}\xspace}
\def\pvalueAGammaRSfits {{\ensuremath{64\%}}\xspace}
\def\pvalueAGammaRSaverageRaw {{\ensuremath{1 \times 10^{-21}}}\xspace}
\def\pvalueAGammaRSaverageWeightedOne {{\ensuremath{30\%}}\xspace}
\def\pvalueAGammaRSaverage {{\ensuremath{31\%}}\xspace}
\def\pvalueAGammaKKfitsRaw {{\ensuremath{7.4\%}}\xspace}
\def\pvalueAGammaKKfitsWeightedOne {{\ensuremath{42\%}}\xspace}
\def\pvalueAGammaKKfits {{\ensuremath{41\%}}\xspace}
\def\pvalueAGammaKKaverageRaw {{\ensuremath{4 \times 10^{-5}}}\xspace}
\def\pvalueAGammaKKaverageWeightedOne {{\ensuremath{33\%}}\xspace}
\def\pvalueAGammaKKaverage {{\ensuremath{45\%}}\xspace}
\def\pvalueAGammaPPfitsRaw {{\ensuremath{40\%}}\xspace}
\def\pvalueAGammaPPfitsWeightedOne {{\ensuremath{37\%}}\xspace}
\def\pvalueAGammaPPfits {{\ensuremath{31\%}}\xspace}
\def\pvalueAGammaPPaverageRaw {{\ensuremath{0.05\%}}\xspace}
\def\pvalueAGammaPPaverageWeightedOne {{\ensuremath{14\%}}\xspace}
\def\pvalueAGammaPPaverage {{\ensuremath{17\%}}\xspace}

% other results
\def\dilution       {{\ensuremath{(3.1 \pm 0.3)\%}}\xspace}
\def\dilutionRS     {{\ensuremath{(3.08 \pm 0.08)\%}}\xspace}
\def\dilutionKK     {{\ensuremath{(3.5  \pm 0.2 )\%}}\xspace}
\def\dilutionPP     {{\ensuremath{(2.9  \pm 0.5 )\%}}\xspace}
\def\dilutionFactor {1.032 \xspace} % +/- 0.0008
\def\bias       {{\ensuremath{(-0.08 \pm 0.02)\times 10^{-4}}}\xspace}
\def\biasKK     {{\ensuremath{( 0.02 \pm 0.06)\times 10^{-4}}}\xspace}
\def\biasPP     {{\ensuremath{( 0.20 \pm 0.12)\times 10^{-4}}}\xspace}

%%% New commands
%%%%%%%%%%%%%%%%%%%%%%% 

\def\eg     {\textit{e.g.}\xspace}
\def\ie     {\textit{i.e.}\xspace}
\def\versus {\textit{vs.}\xspace}

% Mathematical columns in tables
\newcolumntype{C}{>{$}c<{$}}
\newcolumntype{L}{>{$}l<{$}}
\newcolumntype{R}{>{$}r<{$}}

%% Particles
\def\hp      {{\ensuremath{\hadron^+}}\xspace}
\def\hm      {{\ensuremath{\hadron^-}}\xspace}
\def\hprimem      {{\ensuremath{\hadron^{\prime-}}}\xspace}
\def\hpm     {{\ensuremath{\hadron^\pm}}\xspace}
\def\pispm   {{\ensuremath{\pion^{\pm}_{\mathrm{ \scriptscriptstyle tag}}}}\xspace}
\def\pisp    {{\ensuremath{\pion^{+}_{\mathrm{ \scriptscriptstyle tag}}}}\xspace}
\def\pism    {{\ensuremath{\pion^{-}_{\mathrm{ \scriptscriptstyle tag}}}}\xspace}

%% Decays
\def\KK {{\ensuremath{\Kp\Km  }}\xspace}
\def\PP {{\ensuremath{\pip\pim}}\xspace}
\def\RS {{\ensuremath{\Km\pip }}\xspace}
\def\HH {{\ensuremath{\hm\hp }}\xspace}

\def\DzHH {\decay{\Dz}{\HH}}
\def\DzKK {\decay{\Dz}{\Km\Kp}}
\def\DzPP {\decay{\Dz}{\pim\pip}}
\def\DzRS {\decay{\Dz}{\Km\pip}}
\def\DzWS {\decay{\Dz}{\Kp\pim}}
\def\DzF {\decay{\Dz}{f}}


\def\DzbKK {\decay{\Dzb}{\Kp\Km}}
\def\DzbPP {\decay{\Dzb}{\pip\pim}}
\def\DzbRS {\decay{\Dzb}{\Kp\pim}}
\def\DzbWS {\decay{\Dzb}{\Km\pip}}
\def\DzbF {\decay{\Dzb}{f}}

\def\theDstDzpip{\decay{\theDstarp}{\Dz\pip}}
\def\DstDzpisp  {\decay{\Dstarp}{\Dz\pisp }}
\def\Dzbf {\decay{\Dzb }{\ensuremath{f}}}
\def\fulldecaychain {\decay{\Dstarp}{\Dz(\decay{}{\hp\hm})\pip}}
\def\fulldecaychainpis {\decay{\Dstarp}{\Dz(\decay{}{\hp\hm})\pisp}}

%% Asymmetries
\newcommand{\DY}[1]{{\ensuremath{\Delta Y_{#1}}}\xspace}
\newcommand{\agamma}[1]{{\ensuremath{A_{\Gamma}^{#1}}}\xspace}
%\newcommand{\ycp}[1]{{\ensuremath{y_{\CP}^{#1}}}\xspace}

%% Various
\def\phif   {{\ensuremath{\phi_{\lambda_{f}}}}\xspace}
\def\mhh    {{\ensuremath{m(\HH)}}\xspace}
\def\DstM   {{\ensuremath{m(\Dz\pisp)}}\xspace}

%% Physics
% decay amplitudes
\def\af      {{\ensuremath{A_f}}\xspace}
\def\afb     {{\ensuremath{A_{\bar{f}}}}\xspace}
\def\abf     {{\ensuremath{\bar{A}_f}}\xspace}
\def\abfb    {{\ensuremath{\bar{A}_{\bar{f}}}}\xspace}
\newcommand{\Acpdec}[1]{{\ensuremath{a^{d}_{#1}}}\xspace}
\def\deltakpi  {{\ensuremath{\delta_{K\pi}}}\xspace}

\def\CPV {{\ensuremath{C\!PV}}\xspace}
\def\fdchisq {{\ensuremath{\chi^2_\text{FD}}}\xspace}

% units
\newcommand{\cgev}{\ensuremath{\,c/\nospaceunit{Ge\kern -0.1em V}}\xspace}
\newcommand{\kevcc}{\ensuremath{\aunit{ke\kern -0.1em V\!/}c^2}\xspace}


\newcommand{\approptoinn}[2]{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    #1\propto\cr\noalign{\kern2pt}#1\sim\cr\noalign{\kern-2pt}}}}}

\newcommand{\appropto}{\mathpalette\approptoinn\relax}

\usepackage{floatrow}
\floatsetup[table]{capposition=top}
